The Maximum Cut Problem in Co-bipartite Chain Graphs

A \emph{co-bipartite chain} graph is a co-bipartite graph in which the neighborhoods of the vertices in each clique can be linearly ordered with respect to inclusion. It is known that the maximum cut problem (MaxCut) is NP-Hard in co-bipartite graphs. We consider MaxCut in co-bipartite chain graphs. We first consider the twin-free case and present an explicit solution. We then show that MaxCut is polynomial time solvable in this graph class.

==> figures/TwoPathSetsMeet.tex <==
% Generated with LaTeXDraw 2.0.8
% Sat Mar 21 09:26:32 EET 2015
% \usepackage[usenames,dvipsnames]{pstricks}
% \usepackage{epsfig}
% \usepackage{pst-grad} % For gradients
% \usepackage{pst-plot} % For axes
\scalebox{1} % Change this value to rescale the drawing.
{
\begin{pspicture}(0,-1.5876563)(11.700937,1.5876563)
\definecolor{color509b}{rgb}{0.0,0.0,0.8}
\definecolor{color511b}{rgb}{0.0,0.8,0.2}
\psline[linewidth=0.02cm,fillcolor=black,dotsize=0.07055555cm 2.0]{**-**}(2.0009375,-0.5107812)(5.6009374,-0.5107812)
\psline[linewidth=0.04cm,fillcolor=color509b,dotsize=0.07055555cm 2.0]{-**}(1.2009375,0.28921875)(3.2009375,0.28921875)
\psline[linewidth=0.04cm,fillcolor=color509b,dotsize=0.07055555cm 2.0]{-**}(1.1409374,0.68921876)(4.1009374,0.70921874)
\psline[linewidth=0.04cm,fillcolor=color511b,dotsize=0.07055555cm 2.0]{**-}(3.4009376,0.88921875)(6.2009373,0.88921875)
\psline[linewidth=0.04cm,fillcolor=color511b,dotsize=0.07055555cm 2.0]{**-}(3.6009376,0.48921874)(6.2009373,0.48921874)
\psline[linewidth=0.04cm,fillcolor=color511b,dotsize=0.07055555cm 2.0]{**-}(2.4009376,0.08921875)(6.2009373,0.08921875)
\usefont{T1}{ptm}{m}{n}
\rput(3.8223438,-0.8407813){$S$}
\usefont{T1}{ptm}{m}{n}
\rput(0.91234374,-1.0807812){${\cal P}_u$}
\usefont{T1}{ptm}{m}{n}
\rput(1.7523438,-0.5207813){$u$}
\usefont{T1}{ptm}{m}{n}
\rput(5.8123436,-0.5207813){$v$}
\usefont{T1}{ptm}{m}{n}
\rput(6.552344,-1.0807812){${\cal P}_v$}
\psline[linewidth=0.04cm,fillcolor=color509b,dotsize=0.07055555cm 2.0]{-**}(1.2009375,1.0892187)(5.2009373,1.0892187)
\psline[linewidth=0.04cm,fillcolor=color511b,dotsize=0.07055555cm 2.0]{**-}(4.6009374,1.2892188)(6.2009373,1.2892188)
\psline[linewidth=0.04cm,fillcolor=color511b,dotsize=0.07055555cm 2.0]{**-}(2.8009374,-0.31078124)(6.2009373,-0.31078124)
\usefont{T1}{ptm}{m}{n}
\rput(0.8623437,1.1992188){$P_i$}
\usefont{T1}{ptm}{m}{n}
\rput(0.8723438,0.7992188){$P_j$}
\usefont{T1}{ptm}{m}{n}
\rput(0.91234374,0.39921874){$P_k$}
\psellipse[linewidth=0.04,dimen=outer](11.110937,-0.34078124)(0.47,0.63)
\psellipse[linewidth=0.04,dimen=outer](11.100938,-0.07078125)(0.6,0.9)
\psellipse[linewidth=0.04,dimen=outer](11.100938,0.22921875)(0.6,1.2)
\usefont{T1}{ptm}{m}{n}
\rput(11.122344,-0.10078125){$N(k)$}
\usefont{T1}{ptm}{m}{n}
\rput(11.122344,0.45921874){$N(j)$}
\usefont{T1}{ptm}{m}{n}
\rput(11.092343,1.0592188){$N(i)$}
\usefont{T1}{ptm}{m}{n}
\rput(6.5823436,1.3992188){$P_a$}
\usefont{T1}{ptm}{m}{n}
\rput(6.592344,0.99921876){$P_b$}
\usefont{T1}{ptm}{m}{n}
\rput(6.5823436,0.5992187){$P_c$}
\usefont{T1}{ptm}{m}{n}
\rput(6.592344,0.19921875){$P_d$}
\usefont{T1}{ptm}{m}{n}
\rput(6.5823436,-0.20078126){$P_e$}
\psdots[dotsize=0.12](8.160937,0.86921877)
\psdots[dotsize=0.12](8.160937,0.46921876)
\psdots[dotsize=0.12](8.160937,0.06921875)
\psdots[dotsize=0.12](9.160937,1.0692188)
\psdots[dotsize=0.12](9.160937,0.6692188)
\psdots[dotsize=0.12](9.160937,0.26921874)
\psdots[dotsize=0.12](9.160937,-0.13078125)
\psdots[dotsize=0.12](9.160937,-0.53078127)
\usefont{T1}{ptm}{m}{n}
\rput(7.822344,0.9192188){$i$}
\usefont{T1}{ptm}{m}{n}
\rput(7.8323436,0.51921874){$j$}
\usefont{T1}{ptm}{m}{n}
\rput(7.8723435,0.11921875){$k$}
\usefont{T1}{ptm}{m}{n}
\rput(9.562344,1.0392188){$a$}
\usefont{T1}{ptm}{m}{n}
\rput(9.572344,0.63921875){$b$}
\usefont{T1}{ptm}{m}{n}
\rput(9.562344,0.23921876){$c$}
\usefont{T1}{ptm}{m}{n}
\rput(9.572344,-0.16078125){$d$}
\usefont{T1}{ptm}{m}{n}
\rput(9.562344,-0.56078124){$e$}
\psline[linewidth=0.04cm](8.160937,0.86921877)(9.160937,1.0692188)
\psline[linewidth=0.04cm](8.160937,0.86921877)(9.160937,0.6692188)
\psline[linewidth=0.04cm](8.160937,0.86921877)(9.160937,0.26921874)
\psline[linewidth=0.04cm](8.160937,0.86921877)(9.160937,-0.13078125)
\psline[linewidth=0.04cm](8.160937,0.86921877)(9.160937,-0.53078127)
\psline[linewidth=0.04cm](8.160937,0.46921876)(9.160937,0.6692188)
\psline[linewidth=0.04cm](8.160937,0.46921876)(9.160937,0.26921874)
\psline[linewidth=0.04cm](8.160937,0.46921876)(9.160937,-0.13078125)
\psline[linewidth=0.04cm](8.160937,0.46921876)(9.160937,-0.53078127)
\psline[linewidth=0.04cm](8.160937,0.06921875)(9.160937,-0.13078125)
\psline[linewidth=0.04cm](8.160937,0.06921875)(9.160937,-0.53078127)
\usefont{T1}{ptm}{m}{n}
\rput(3.5860937,-1.3607812){(a)}
\usefont{T1}{ptm}{m}{n}
\rput(8.956094,-1.3607812){(b)}
\usefont{T1}{ptm}{m}{n}
\rput(11.086094,-1.3607812){(c)}
\end{pspicture} 
}



==> figures/optimalcut.tex <==
% Generated with LaTeXDraw 2.0.8
% Wed Mar 11 16:43:43 EET 2015
% \usepackage[usenames,dvipsnames]{pstricks}
% \usepackage{epsfig}
% \usepackage{pst-grad} % For gradients
% \usepackage{pst-plot} % For axes
\scalebox{1} % Change this value to rescale the drawing.
{
\begin{pspicture}(0,-1.45375)(5.0428123,1.41375)
\psframe[linewidth=0.02,dimen=outer](3.8609376,1.41375)(3.4609375,-0.98625)
\psframe[linewidth=0.02,dimen=outer,fillstyle=solid,fillcolor=black](4.8609376,1.41375)(4.4609375,-0.98625)
\psframe[linewidth=0.02,dimen=outer,fillstyle=solid,fillcolor=black](3.8609376,0.61375)(3.4609375,-0.98625)
\psframe[linewidth=0.02,dimen=outer,fillstyle=solid](4.8609376,1.41375)(4.4609375,-0.18625)
\psline[linewidth=0.02cm,linestyle=dashed,dash=0.16cm 0.16cm](4.8609376,0.61375)(1.2609375,0.61375)
\psline[linewidth=0.02cm,linestyle=dashed,dash=0.16cm 0.16cm](4.8609376,-0.18625)(1.2609375,-0.18625)
\usefont{T1}{ptm}{m}{n}
\rput(3.6123438,-1.27625){$K$}
\usefont{T1}{ptm}{m}{n}
\rput(4.6523438,-1.27625){$K'$}
\usefont{T1}{ptm}{m}{n}
\rput(2.1123438,1.00375){$\approx \frac{\abs{K}}{3}$}
\usefont{T1}{ptm}{m}{n}
\rput(2.1123438,0.12375){$\approx \frac{\abs{K}}{3}$}
\usefont{T1}{ptm}{m}{n}
\rput(2.1123438,-0.61625){$\approx \frac{\abs{K}}{3}$}
\end{pspicture} 
}


